AIMSCheck: Leveraging LLMs for AI-Assisted Review of Modern Slavery Statements Across Jurisdictions

Modern Slavery Acts mandate that corporations disclose their efforts to combat modern slavery, aiming to enhance transparency and strengthen practices for its eradication. However, verifying these statements remains challenging due to their complex, diversified language and the sheer number of statements that must be reviewed. The development of NLP tools to assist in this task is also difficult due to a scarcity of annotated data. Furthermore, as modern slavery transparency legislation has been introduced in several countries, the generalizability of such tools across legal jurisdictions must be studied. To address these challenges, we work with domain experts to make two key contributions. First, we present AIMS.uk and AIMS.ca, newly annotated datasets from the UK and Canada to enable cross-jurisdictional evaluation. Second, we introduce AIMSCheck, an end-to-end framework for compliance validation. AIMSCheck decomposes the compliance assessment task into three levels, enhancing interpretability and practical applicability. Our experiments show that models trained on an Australian dataset generalize well across UK and Canadian jurisdictions, demonstrating the potential for broader application in compliance monitoring. We release the benchmark datasets and AIMSCheck to the public to advance AI-adoption in compliance assessment and drive further research in this field.

==> Sector.tex <==
\subsection{Sector}

We categorize industries into four broad sectors: 
Industry \& Infrastructure, Commerce \& Services, Public \& Healthcare, and Other. 

\begin{enumerate}
    \item The Industry \& Infrastructure sector includes industries such as automotive, construction, durable consumer goods, mining, utilities, waste management, transportation, defense, and security services.
    \item The Commerce \& Services sector covers consumer services, including hospitality, tourism, fashion, cosmetics, food and agriculture, finance, professional services, IT, and media.
    \item The Public \& Healthcare sector consists of public sector organizations, non-profits, education, healthcare, and forestry-related industries.
    \item The Other category represents industries that do not fit into these three sectors.
\end{enumerate}

In terms of company distribution, Industry \& Infrastructure accounts for 35 companies, Commerce \& Services includes 31, Public \& Healthcare comprises 9, and Other consists of 13 companies.

We summarize the proportion of companies in each sector that comply with specific criteria. The statistics are shown in Table~\ref{fig:turnover-sector}

\begin{table}[]
\begin{tabular}{|c|c|}
\hline
Sector                     & Number of Statement \\ \hline
Commerce \& Services       & 17                  \\ \hline
Industry \& Infrastructure & 20                  \\ \hline
 Public \& Healthcare       & 5                   \\ \hline
 Other                      & 8                   \\ \hline
\end{tabular}
\caption{Compliance Proportion by Sector for Each Criterion}
\label{fig:turnover-sector}
\end{table}

\begin{figure*}
    \centering
     \includegraphics[width=\textwidth]{images/compliance_proportion_sector_appendix.png}
    \caption{Compliance Proportion by Sector for Each Criterion}
    \label{fig:sector-apd}
 \end{figure*}

  Figure~\ref{fig:sector-apd} shows the compliance proportion by sector for each criterion.

  \textbf{Key Observations}
